Dynamical Phenomena on Complex Networks

The work presented in this thesis concerns different aspects of dynamical processes on networks. The first subject considered is the theoretical modeling of exploration processes of complex networks, such as the ``traceroute'' process used to map the Internet. Our mean-field analysis of the traceroute model provides a better understanding of the Internet topology. A second part of the thesis is devoted to the study of the weighted representation of networks and their relations with the functional properties of infrastructure systems (e.g. the airports network). Other results concerning spreading processes and percolation on weighted networks are presented. Finally, we turns to social networks, introducing the Naming Game, a model for the emergence of a communication system in a structured population of individuals. We show that the dynamical phenomena generated by this model depend strongly on the topology of the interactions.

==> App4_3.tex <==
\chapter{Generating Functions in Percolation Problems}
\label{APP4_1}

In this Appendix, we provide a brief introduction to the formalism of generating functions in the study of percolation on random graphs. We consider infinite graphs without isolated vertices, and self-edge or multiple edges. 
The generating function for the degree distribution $p_k$ of a randomly chosen vertex is
\begin{equation}
G_{0}(x)=\sum_{k=1}^{\infty}p_{k}x^{k}~,
\end{equation}
with $G_{0}(1)=1$, and $\langle k \rangle =\sum_{k}k p_{k} = G_{0}'(1)$. 
Similarly, the generating function for the probability that a randomly chosen edge leads to a vertex of given degree is
\begin{equation}
\frac{\sum_{k}k p_{k} x^{k-1}}{\sum_{k}k p_{k}} = G_{1}(x)= \frac{G_{0}'(x)}{G_{0}'(1)}~.
\end{equation}
A useful property is that the probability distribution and its moments can be computed by simple derivative of the corresponding generating function. 

If we call $q_{k}$ the probability that a vertex of degree $k$ is occupied (or node traversing probability if regarded as a spreading phenomena), the probability that, choosing randomly a vertex, we pick up an occupied vertex of degree $k$ is the product of the probabilities of two independent events, i.e. $p_{k}q_{k}$. Repeating the same operation with the edges, we need the probability that the randomly chosen edge is attached to an occupied vertex of degree $k$. This event happens with probability $k p_{k} q_{k} /\langle k \rangle$.  
Hence, we define the generating functions for both these probabilities that are very important in the site percolation,
\begin{subequations}
\begin{align}
 F_{0}(x; \{q\})& =\sum_{k=1}^{\infty}p_{k} q_{k} x^{k}~,\label{f0}\\
 F_{1}(x; \{q\})& =\frac{\sum_{k=1}^{\infty} k p_{k} q_{k} x^{k-1}}{\sum_{k}k p_{k}} = \frac{F_{0}'(x)}{\langle k\rangle}~.\label{f1}
 \end{align}
\end{subequations}
The function $F_{0}(x; \{q\})$ is the generating function of the probability that a vertex of a given degree exists and is occupied, while $F_{1}(x; \{q\})$ is the generating function for the probability of reaching a vertex of a given degree starting by a randomly chosen edge and that it is occupied.

The solution of the site percolation problem is the set of values $\{q_k\}$ for which an infinite cluster (giant component) exists. 
In order to compute the probability that a randomly chosen vertex belongs to the giant component, we start by computing the probability $P_{s}$ that a randomly chosen vertex belongs to a connected cluster of a certain size $s$. 
The use of generating functions allows to do it simultaneously for all the possible sizes. Then, the mean cluster size is obtained as the first derivative of the generating function of $P_{s}$. 
Finally, the condition for the divergence of the mean cluster size gives the condition for the existence of the giant component as a function of the parameters of the system, that are the degree distribution and the node occupation probability.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[thb] 
\centerline{
\begin{tabular}{|c|}\hline \\ \includegraphics*[angle=-90,width=0.45\textwidth]{FIG/vul_perc/gene1}\\ \hline\end{tabular}~~
\begin{tabular}{|c|}\hline \\ \includegraphics*[angle=-90,width=0.45\textwidth]{FIG/vul_perc/gene0}\\ \hline\end{tabular}
}
%
\caption{A) A full dotted bullet with dashed contour line corresponds to the probability that a vertex is unoccupied. This is given by a particular series of diagrams, in which we sum the contributions of unoccupied vertices of all possible degrees.  
A striped bullet with full contour line represents the generating function $F_{0}(x;\{q\})$, whose diagrammatical expansion
contains all possible combinations of occupied vertices reachable by an occupied vertex with a certain degree. The $x$ accounts for the occupation of a vertex. 
The contributions of the isolated vertices ($p_{0}q_{0}$) have been deleted in agreement with our convention of considering only graphs with non isolated vertices.  
B) Diagrammatical representation of the generating function $H_{0}(x)$. The first terms of the infinite series correspond to the summation of the Eqs.~\ref{series} as presented in Eq.~\ref{lungaH0}. These contributions can be expressed in a compact form using Eq.~\ref{h00}, that contains the  generating functions $F_{0}(x;\{q\})$ and $H_{1}(x)$.\\}
\label{diag1}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%

Firstly, we consider the probability $P_{s}$ that a randomly chosen vertex in the network belongs to a connected cluster of a certain size $s$. We call $H_{0} (x; \{q\})$ its generating function,
\begin{equation}
H_{0}(x; \{q\}) = \sum_{s=0}^{\infty} P_{s} x^{s}~,
\end{equation}
in which we have conventionally grouped in the term for $s=0$ the probability $1-\sum_{k}q_{k}p_{k}$ that a vertex is not occupied.
Similarly, let $\hat{P_{s}}$ be the probability that a randomly chosen edge leads to a cluster of a given size $s$, and $H_{1}(x; \{q\})$  its generating function. 
  
Since we choose the starting vertex at random, each possible degree $k$ gives a different contribution to each possible cluster size probability $P_{s}$, meaning that each term $P_{s} x^{s}$ is itself given by an infinite sum of terms labeled by the degree $k$. 
For instance, the first terms of $H_{0}(x; \{q\})$ are:
\begin{subequations}\label{series}
\begin{align}
 P_{0}~~& = 1 - \sum_{k} p_{k} q_{k}~,\label{ser1}\\
 P_{1}x~& = \sum_{l=1}^{\infty} {p_{l} q_{l} x ~\hat{P_{0}}}^{l}~,\label{ser2}\\
 P_{2}{x}^{2}& = \sum_{l=1}^{\infty} {l p_{l} q_{l} x ~(\hat{P_{1}} x)}~{\hat{P_{0}}}^{l-1}~,\label{ser3}\\
 P_{3}{x}^{3}& = \sum_{l=1}^{\infty} {l p_{l} q_{l} x ~(\hat{P_{2}} {x}^{2})~\hat{P_{0}}^{l-1}} + \sum_{l\geq 2} p_{l} q_{l} x ~{\left(\begin{array}{c} l\\ 2\end{array}\right)}~{(\hat{P_{1}} x)}^{2}~\hat{P_{0}}^{l-2}~,\label{ser4}\\
 P_{4}{x}^{4}& = \sum_{l=1}^{\infty} l p_{l} q_{l} x ~(\hat{P_{3}} {x}^{3})~{\hat{P_{0}}}^{l-1} + \sum_{l\geq 2} p_{l} q_{l} x ~2 {\left(\begin{array}{c} l \\ 2 \end{array} \right)}~{(\hat{P_{2}} x^2)}~(\hat{P_{1}} x)~{\hat{P_{0}}}^{l-2}\\ \quad & \quad\quad +\sum_{l\geq 3} p_{l} q_{l} x ~{\left(\begin{array}{c} l \\ 3 \end{array} \right)}~{(\hat{P_{1}} x)}^3~{\hat{P_{0}}}^{l-3}~,\label{ser5}\\
\nonumber ~& \vdots
\end{align}
\end{subequations}
Now, summing these terms and grouping similar contributions we get
\begin{equation}\label{lungaH0}
\begin{split} H_{0}(x; \{q\})& = 1 - \sum_{k} p_{k} q_{k} + p_{1} q_{1} x ~ \left[ \hat{P_{0}} + \hat{P_{1}} x + \hat{P_{2}} {x}^{2} + \dots \right] \\
&\quad\quad + p_{2} q_{2} x ~ \left[ {\hat{P_{0}}}^{2} + 2 \hat{P_{0}} ~\hat{P_{1}} x + {(\hat{P_{1}} x)}^{2} + 2 \hat{P_{0}} ~\hat{P_{2}} x^{2} \\ 
&\quad\quad\quad + 2 \hat{P_{1}} x ~ \hat{P_{2}} {x}^{2} + {(\hat{P_{2}} {x}^{2})}^{2} + \dots \right] + \dots \\
&= 1 - \sum_{k} p_{k} q_{k}  + p_{1} q_{1} x \left[ \hat{P_{0}} + \hat{P_{1}} x +  \hat{P_{2}} {x}^{2} + \dots \right]\\ 
&\quad\quad+ p_{2} q_{2} x ~{\left[ \hat{P_{0}} + \hat{P_{1}} x +  \hat{P_{2}} {x}^{2} + \dots \right]}^{2} + \dots~\\
&= 1 - \sum_{k} p_{k} q_{k}  + x p_{1} q_{1} H_{1}(x; \{q\}) + x p_{2} q_{2} {\left[ H_{1}(x; \{q\})\right]}^{2} + \dots~.
\end{split}
\end{equation}
Note that no term contains $p_{0}q_{0}$ according with the convention of considering only non isolated nodes.
A compact form for this expression is written using Eq.~\ref{f0},
\begin{eqnarray}
H_{0}(x; \{q\}) = 1-F_{0}(1;\{q\}) + x F_{0}(H_{1}(x; \{q\}); \{q\})~.
\label{h00}
\end{eqnarray}
The structure of Eq.~\ref{h00} can be represented diagrammatically as shown in Fig.~\ref{diag1}, associating the variable $x$ to each ``bare'' vertex and a variable $H(x; \{q\})$ to each ``dressed'' vertex, while the function $F_{0}$  weights the contributions over all possible degrees.  

Moreover, the generating function $H_{1}(x; \{q\})$ satisfies a similar self-consistent equation,
\begin{eqnarray}
H_{1}(x; \{q\}) = 1-F_{1}(1;\{q\}) + x F_{1}(H_{1}(x; \{q\}); \{q\})~,
\label{h01}
\end{eqnarray}
that is obtained following completely similar arguments starting from picking up an edge at random. 

Taking the first derivative of $H_{0}$ in Eq.~\ref{h00} with respect to $x$ computed in $x=1$, we get the mean cluster size $\langle s \rangle$. Then, imposing the divergence of the latter allows to find the condition for the existence of a giant component, that corresponds to the Molloy-Reed criterion as presented in Ref.~\cite{callaway}. Finally, considering a uniform occupation probability $q_{k}=q$ (or uniform node traversing probability), the expression for the site percolation threshold $q_{c}$ can be computed. 



==> App5_3.tex <==
\chapter{The origin of the effective surface tension: modified Voter model}\label{APP5_3}

In this appendix, we report some preliminary result about the origin of the effective surface tension
generated by the Naming Game's evolution rules [REF]. 
The convergence properties of the Naming Game are, indeed, very similar to those of non-equilibrium models based on a majority rule, i.e. Ising-like models.
For any finite dimension $d$, non-equilibrium majority rule models approach the ordered state by means of a diffusive coarsening process, such that the time required to reach the ferromagnetic ground state scales as $N^{2/d}$ with the size $N$ of the system.
This is exactly the scaling law of the Naming Game, apart from a factor $N$ coming from the different time scale (in the Naming Game the temporal step coincides with the single interaction, while in usual statistical mechanics models the time scale consists of $N$ interactions).
The two models present the same scaling law because their dynamics is governed by a similar coarsening process of clusters of sites.    
